Sliding Mode Control of Active Magnetic Bearings -- A Cascaded Architecture

Accurate and robust positioning of rotor axle is essential for efficient and safe operation of high-speed rotational machines with active magnetic bearings. This study presents a cascaded nonlinear control strategy for vertical axial positioning of an active magnetic bearing system. The proposed scheme employs two sliding mode controllers for regulating rotor vertical position and current and an adaptive estimator to invert the nonlinear input mapping. Uniform asymptotic stability is proven for the closed-loop system and the efficacy and performance of the proposed design is evaluated in simulation.

==> Tables/des_tab.tex <==
\begin{tabular*}{1.0\columnwidth}{@{\extracolsep\fill}clc@{\extracolsep\fill}}	
	\toprule%{clc}
	\multicolumn{1}{l}{\textbf{Symbol}}	& \multicolumn{1}{l}{\textbf{Description}} & \multicolumn{1}{c}{\textbf{Value}}\T\B \\
	\specialrule{.2em}{.1em}{-1em}\\
	\multicolumn{3}{l}{\textbf{Rotor axial control parameters}}\T\B \\\hline
	$A$ 	& Cross-sectional area 		& $275$\T\B \\\hline
	\multicolumn{3}{l}{\textbf{Input estmators parameters}}\T\B \\\hline
	$s_0$ 	& Air gap size 				& $5\cdot 10^5$\T\B \\
	$i_0$ 	& Bias current				& $10^4$\T\B \\
	$R$ 	& Coil resistance			& $0.2 \; \si{\radian\per\second}$\T\B \\
	$\gamma$& Adaptation gain			& $0.5$\T\B \\
	$g$ 	& gravitational acceleration& $\left[ 0.15, 0.15, 0.005 \right]$\T\B \\
	\multicolumn{3}{l}{\textbf{Current controller parameters}}\T\B \\\hline
	$c$		& $z$ decay rate			& $0.008 \; \si{\newton\meter}$\T\B \\
	$k$ 	& $z$ \gls{SMC} gain 		& $1.25 \; \si{\newton\meter}$\T\B \\
	$k_i$	& $i$ \gls{SMC} gain		& $\left[ 0.008, 0.008, 0.01 \right]^T$\T\B \\\hline
\end{tabular*}
